SplitMeanFlow: Interval Splitting Consistency in Few-Step Generative Modeling

Generative models like Flow Matching have achieved state-of-the-art performance but are often hindered by a computationally expensive iterative sampling process. To address this, recent work has focused on few-step or one-step generation by learning the average velocity field, which directly maps noise to data. MeanFlow, a leading method in this area, learns this field by enforcing a differential identity that connects the average and instantaneous velocities. In this work, we argue that this differential formulation is a limiting special case of a more fundamental principle. We return to the first principles of average velocity and leverage the additivity property of definite integrals. This leads us to derive a novel, purely algebraic identity we term Interval Splitting Consistency. This identity establishes a self-referential relationship for the average velocity field across different time intervals without resorting to any differential operators. Based on this principle, we introduce SplitMeanFlow, a new training framework that enforces this algebraic consistency directly as a learning objective. We formally prove that the differential identity at the core of MeanFlow is recovered by taking the limit of our algebraic consistency as the interval split becomes infinitesimal. This establishes SplitMeanFlow as a direct and more general foundation for learning average velocity fields. From a practical standpoint, our algebraic approach is significantly more efficient, as it eliminates the need for JVP computations, resulting in simpler implementation, more stable training, and broader hardware compatibility. One-step and two-step SplitMeanFlow models have been successfully deployed in large-scale speech synthesis products (such as Doubao), achieving speedups of 20x.

==> sections/experiments_old.tex <==
\section{Experiments}

\subsection{Experimental Settings}
Above we focus on the discussion of the principle. Next, we explain the details of our experiment. 

% \textbf{Loss Function Modification:} The loss function in Algorithm~\ref{alg:splitmeanflow_training} assigns a higher training weight to regions with larger time intervals $t-r$ and a lower weight to regions with smaller intervals. To avoid this issue, we introduce the parameter $\delta=\lambda(t-r)$, where $0\le \lambda \le 1$, and let $t-s=\delta=\lambda(t-r)$ and $s-r=(1-\lambda)(t-r)$. Then the identity \ref{eq:interval_splitting_conssitency} becomes
% \begin{equation}
%     u(z_t,r,t) = (1-\lambda)u(z_{t-\delta},r,t-\delta) + \lambda u(z_t,t-\delta,t)
% \label{eq:interval_splitting_conssitency2}
% \end{equation}


\textbf{Boundary Conditions:} The identity \ref{eq:interval_splitting_conssitency3} is a difference equation that must satisfy the following boundary conditions: when $r=t$, then $u(z_t, r, t)=v(z_t, t)$. The same to meanflow, within each batch of training data, we randomly select a proportion $p$ (termed as flow ratio in MeanFlow) of samples, set their $t$ equal to $r$, and assign targets $v(z_t, t)$ to these samples. In practice, we find that the value of $p$ must exceed 0.5 to achieve valid results.

\textbf{Pretraining and Distillation:} Although SplitMeanFlow can be trained from scratch like meanflow, we strongly recommend pretraining to meet industrial deployment standards. During pretraining, we set flow ratio $p=1$, enable CFG~\cite{ho2022classifier} dropout (setting cfg\_dropout=0.1), and train until full convergence is achieved, yielding a standard flow matching model. This model then serves as: (1) the initialization weights for subsequent training of SplitMeanFlow (named as student model), (2) the teacher model providing instantaneous velocity $v(z_t, t)$ with CFG. Empirically, we find that this approach achieves significantly faster convergence and superior performance compared to from scratch training and sample-velocity $\epsilon - x$ supervision. In greater technical detail, when training with SplitMeanFlow, cfg\_dropout is set 0.0. For each batch of training data, we first generate targets (defined in Algorithm~\ref{alg:splitmeanflow_training}) in evaluation mode (disabling all dropout and data augmentation), then execute forward-backward propagation in training mode.




% \subsection{Private Experiments}
We conducted extensive evaluations of SplitMeanFlow Text-to-Speech (TTS) task on Seed-TTS~\cite{anastassiou2024seed}. Seed-TTS contains four blocks: a speech tokenizer, a token language model, a token diffusion model, and an acoustic vocoder. In all of our private experiments, all blocks except the diffusion model were pre-trained on a massive training set, thus fixing their parameters. We only train the diffusion model. The diffusion model contains 24 transformer layers, totaling around 400 million parameters. We employ a combined pretraining and distillation strategy. First, the model undergoes extensive pretraining following the standard flow matching paradigm until it can generate high-quality speech via multi-step decoding and CFG. This pretrained model then serves dual roles—as initialization weights and teacher—for training SplitMeanFlow. We introduce two of the scenarios we apply: 1. Zero-shot in-context learning (ICL), 2. Speaker fine-tuning (SFT) defined in Seed-TTS~\cite{anastassiou2024seed}.

\textbf{In-context learning: } In this task, each sample of training data contains one reference utterance and one target utterance spoken by the same speaker, and the model is trained to generate speech of the target text based on the reference speech as an audio prompt. During inference, given any piece of text and any audio prompt, we hope that the model can generate a speech of the text with the timbre given by the audio prompt.

\textbf{Speaker fine-tuning: } After sufficient training in the ICL scenario, we continue to fine-tune on a fixed timbre using some high-quality corpus. During inference, only a piece of text needs to be given, and the model is required to output speech of the target text with this fixed timbre.



Our algorithm achieves speech quality on par with the NFE=10 enabling CFG configuration under significantly reduced settings (NFE=1 or 2, with out CFG) in TTS tasks. This is validated by a Comparative Mean Opinion Score (CMOS) score of -0.01 and has been deployed on Doubao. This work establishes the first known industrial implementation with NFE $\le$ 2, a landmark in efficient generative modeling for speech synthesis.







% \subsection{Public Experiments}

